RiskBench: A Scenario-based Benchmark for Risk Identification

Intelligent driving systems aim to achieve a zero-collision mobility experience, requiring interdisciplinary efforts to enhance safety performance. This work focuses on risk identification, the process of identifying and analyzing risks stemming from dynamic traffic participants and unexpected events. While significant advances have been made in the community, the current evaluation of different risk identification algorithms uses independent datasets, leading to difficulty in direct comparison and hindering collective progress toward safety performance enhancement. To address this limitation, we introduce \textbf{RiskBench}, a large-scale scenario-based benchmark for risk identification. We design a scenario taxonomy and augmentation pipeline to enable a systematic collection of ground truth risks under diverse scenarios. We assess the ability of ten algorithms to (1) detect and locate risks, (2) anticipate risks, and (3) facilitate decision-making. We conduct extensive experiments and summarize future research on risk identification. Our aim is to encourage collaborative endeavors in achieving a society with zero collisions. We have made our dataset and benchmark toolkit publicly on the project page: https://hcis-lab.github.io/RiskBench/

==> Content/xxx.tex <==
\section*{\LARGE Appendix}
In this appendix, we cover,
\begin{enumerate}[label=\Alph*)]

\item Details of scenario collection

\item nuScenes annotation

\item More ablation study of Action-slot

\item Analysis in challenging scenarios

\item Limitations

\item Implementation details

\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[t!]
    \scriptsize
    \centering
    \caption{\textbf{Risk identification results in risk types.} The numbers reported are F1 scores. }      %%%%%% interactive+collision
    \begin{tabular}
            {@{}l@{\;} @{\;} @{\;} c @{\;}@{\;}@{\;} @{\;}@{\;}@{\;}c @{\;}@{\;}@{\;} @{\;}@{\;}@{\;} c @{\;}@{\;}@{\;} @{\;}@{\;}@{\;} c @{\;}}
            
            \toprule
             \multirow{1}{*}{ \begin{tabular}{@{\;}c@{\;}} \end{tabular}} & 
             \multicolumn{1}{c}{Four-wheeler }  & 
             \multicolumn{1}{c}{Two-wheeler }  & 
             \multicolumn{1}{c}{Pedestrian}   & 

             \\
             \toprule
             % Kalman Filter~\cite{thrun2002probabilistic}
             %  &  &  &  \\
             % Social-GAN~\cite{social-gan}   
             %  &  & &  \\
             % MANTRA~\cite{mantra}
             %  &  &  & 
             %  \\
             QCNet~\cite{zhou2023query}
             & 57.2 & 61.5 & 14.3
             \\
             
             \midrule
             RRL~\cite{zeng2017agent}
             & 44.5 & 62.6 & 64.3
             \\
             BCP~\cite{li2020make}
             & 44.2 & 21.4 & 29.1 
             \\
             
             \midrule
             RRL+state
             & 59.1 & 62.7 & 69.2
             \\
             BCP+state
             & 55.2 & 34.6 & 42.2
             \\

             \midrule
            \bottomrule
        \end{tabular}
        \label{table:agent_type}

\end{table}


\begin{table}[t!]
\centering
\caption{The statistics of the training, validation, and testing sets in different scenario types.}
\small
        \begin{tabular}{ccccc}
             \toprule
             \multirow{1}{*}{ \begin{tabular}{@{\;}c@{\;}} \end{tabular}} & 
             \multicolumn{1}{c}{Interactive}  & 
             \multicolumn{1}{c}{Collision }  & 
             \multicolumn{1}{c}{Obstacle}   & 
             \multicolumn{1}{c}{Non-inter.}   & 
            \toprule
            Training    & 925 & 1044 & 850 & 1023
            \\
            \midrule
            Validation  & 348 & 283 & 258 & 496
            \\
             \midrule
            Testing     & 521 & 375 & 322 & 471
            \\
             \midrule
             \bottomrule

        \end{tabular}
        \label{tab:datasplit}

\end{table}


\begin{table*}[t!]
\centering
\small
        \begin{tabular}{cc}
             \toprule
             % \multirow{1}{*}{ \begin{tabular}{@{\;}c@{\;}} \end{tabular}} & 
             \multicolumn{1}{c}{\textbf{Attribute}}  &
             \multicolumn{1}{c}{\textbf{Value}}  &
            \toprule
            Map    & Town01, Town02, Town03, Town05, Town06, Town07, Town10HD, A0, A1, A6, B3, B7, B8
            \\
            \midrule
            Road topology  & forward, left turn, right turn, u-turn, lane change left, right lane change
            \\
             \midrule
            Interaction type & interactive, collision, obstacle, non-interactive
            \\
             \midrule
            Interacting agent type & car, truck, bicyclist, motorcyclist, pedestrian
            \\
             \midrule
            Interacting agent's behavior & \makecell{ forward, left turn, right turn, u-turn, lane change left, right lane change, crosswalking, \\ jaywalking, go into roundabout, go around roundabout, exit roundabout}
            \\
             \midrule
            Obstacle type & traffic cone, barrier, warning, illegal parking vehicle
            \\
             \midrule
            Traffic violation & Running red light, ignoring stop sign, driving on sidewalk, jay-walker
            \\
             \midrule
            Ego's reaction & right-deviation, left-deviation
            \\
             \midrule
             \bottomrule

        \end{tabular}
        \label{tab:taxonomy}
\caption{Scenario Taxonomy}

\end{table*}


\begin{table*}[t!]
    \scriptsize
    \centering
\caption{\textbf{Temporal Consistency} results calculated within 1, 2, and 3 seconds before the critical/collision point. \hank{we can add a new experiments that tests if filter can help planning-awareness evaluation. A simple way is to use random to disturb the consistency.}}       %%%%%% interactive+obstacle+collision
\begin{tabular}
            {@{}l @{\;}@{\;}@{\;} c @{\;}@{\;}@{\;}  c @{\;}@{\;}@{\;}  c @{\;}@{\;}@{\;}  c @{\;}@{\;}@{\;}  c @{\;}@{\;}@{\;}  c @{\;}@{\;}@{\;} c @{\;}@{\;} @{\;} c @{\;} c @{\;}@{\;}@{\;} c @{\;}@{\;} c @{\;}@{\;}@{\;} c @{\;}@{\;}@{\;}}
            \toprule
            \multirow{2}{*}{ \begin{tabular}{@{\;}c@{\;}} \end{tabular}} & 
             \multicolumn{3}{@{\;}c}{consistency}  & 
             % \multicolumn{1}{@{\;}c}{2s}  & 
             % \multicolumn{1}{@{\;}c}{3s}   & 
             \multicolumn{1}{@{\;}c}{P}   & 
             \multicolumn{1}{@{\;}c}{R}   & 
             \multicolumn{1}{@{\;}c}{F1}   & 
             \multicolumn{1}{@{\;}c}{PIC}   & 
             \multicolumn{2}{@{\;}c@{\;}}{interactive}   & 
             \multicolumn{2}{@{\;}c@{\;}}{obstacle}   & 

             \\
             \cmidrule(lr){2-4}
             \cmidrule(lr){9-10} 
             \cmidrule(lr){11-12}
             &
             \multicolumn{1}{@{\;}c}{1s}&
             \multicolumn{1}{@{\;}c}{2s}&
             \multicolumn{1}{@{\;}c}{3s}& 
              & & & & 
             \begin{tabular}{@{\;}@{\;}c@{\;}}  IR  \end{tabular} & 
             \begin{tabular}{@{\;}c@{\;}}  CR (\%)  \end{tabular} & 
             \begin{tabular}{@{\;}@{\;}c@{\;}}  IR   \end{tabular} & 
             \begin{tabular}{@{\;}c@{\;}}  CR (\%)  \end{tabular} & 
            
             \\
             \toprule
             RRL~\cite{zeng2017agent}
             & 19.0 & 8.5 & 4.8 & 72.8 & 38.0 & 49.9 & 15.3 & 0.01 & 1.2 & 0.49 & 54.3
             \\
             RRL+smoothing % threshold===0.25
             & 54.7 & 36.3 & 25.7 & 48.6 & 64.6 & 55.4 & 10.1 & 0.03 & 1.5 & 0.39 & 41.8
             \\

             \midrule
             BCP~\cite{li2020make}
             & 7.0 & 3.9 & 3.4  & 48.3 & 26.5 & 34.2 & 22.2 & 0.14 & 9.7 & 0.34 & 39.4
             \\
             BCP+smoothing % threshold===0.18
             & 11.7 & 7.5 & 6.6 & 33.2 & 31.6 & 32.4 & 20.7 & 0.14 & 1.2 & 0.27 & 30.3
             \\
             
              \midrule
            \bottomrule
        \end{tabular}
        
\label{table:consistency}
\end{table*}



\begin{table*}[t!]
    \scriptsize
    \centering
\caption{\textbf{Temporal Consistency} results calculated within 1, 2, and 3 seconds before the critical/collision point. \hank{we can add a new experiments that tests if filter can help planning-awareness evaluation. A simple way is to use random to disturb the consistency.}}       %%%%%% interactive+obstacle+collision
\begin{tabular}
            {@{}l @{\;}@{\;}@{\;} c @{\;}@{\;}@{\;}  c @{\;}@{\;}@{\;}  c @{\;}  c @{\;}  c @{\;}@{\;}@{\;}  c @{\;} c @{\;}@{\;} @{\;} c}
            \toprule
            \multirow{2}{*}{ \begin{tabular}{@{\;}c@{\;}} \end{tabular}} & 
             \multicolumn{3}{@{\;}c}{consistency}  & 

             \multicolumn{2}{@{\;}c@{\;}}{interactive}   & 
             \multicolumn{2}{@{\;}c@{\;}}{obstacle}   & 

             \\
             \cmidrule(lr){2-4}
             \cmidrule(lr){5-6} 
             \cmidrule(lr){7-8}
             &
             \multicolumn{1}{@{\;}c}{1s}&
             \multicolumn{1}{@{\;}c}{2s}&
             \multicolumn{1}{@{\;}c}{3s}& 
              
             \begin{tabular}{c@{\;}@{\;}@{\;}}  IR  \end{tabular} & 
             \begin{tabular}{c@{\;}@{\;}}  CR (\%)  \end{tabular} & 
             \begin{tabular}{c@{\;}@{\;}@{\;}}  IR   \end{tabular} & 
             \begin{tabular}{c@{\;}@{\;}}  CR (\%)  \end{tabular} & 
            
             \\
             \toprule
             RRL~\cite{zeng2017agent}
             & 19.0 & 8.5 & 4.8 & 0.01 & 1.2 & 0.49 & 54.3
             \\
             RRL+smoothing % threshold===0.25
             & 54.7 & 36.3 & 25.7 & 0.03 & 1.5 & 0.39 & 41.8
             \\

             \midrule
             BCP~\cite{li2020make}
             & 7.0 & 3.9 & 3.4  & 0.14 & 9.7 & 0.34 & 39.4
             \\
             BCP+smoothing % threshold===0.18
             & 11.7 & 7.5 & 6.6 & 0.14 & 1.2 & 0.27 & 30.3
             \\
             
              \midrule
            \bottomrule
        \end{tabular}
        
\end{table*}



% --------------
% \subsection{Fine-grained Scenario-based Evaluation}
\label{subsec:fine-grained}
\begin{table*}[t!]
    \small
    \centering
    % \resizebox{\textwidth}{!}{
        \begin{tabular}
            {@{}l @{\;}@{\;} c @{\;}@{\;} c @{\;} @{\;}  c @{\;}@{\;}   c @{\;}@{\;}  c @{\;}@{\;}   c @{\;}@{\;}  c @{\;}@{\;}  c @{\;}@{\;}  c @{\;}@{\;}  c @{\;}@{\;} }
            \toprule
            \multirow{1}{*} {\begin{tabular}{@{\;}c@{\;}} Risk Id. Algor. \end{tabular}} & 
             % \multicolumn{1}{c}{Night}  & 
             \multicolumn{1}{c}{Rainy}  & 
             \multicolumn{1}{c}{4-way}   & 
             \multicolumn{1}{c}{3-way} &
             \multicolumn{1}{c}{Straight} &
             \multicolumn{1}{c}{TD low} &
             \multicolumn{1}{c}{TD mid} &
             \multicolumn{1}{c}{TD high} &
             \multicolumn{1}{c}{Average} &
             
            \\
             \toprule
             Random
             & 15.2 & 12.5 & 12.7 & 14.5 & 19.3 & 14.2 & 12.9 & 15.1
             \\
             Range (10m) 
             & 53.4 & 45.4 & 44.7 & 52.0 & 57.1 & 52.4 & 51.8 & 53.6
             \\

            \midrule
             Kalman Filter~\cite{thrun2002probabilistic}
             & 46.7 & 38.7 & 37.8 & 44.0 & 52.9 & 44.7 & 43.7 & 46.7
             \\
             Social-GAN~\cite{social-gan}   
             & 45.7 & 33.5 & 37.0 & 46.6 & 50.4 & 44.1 & 44.1 & 46.0
             \\
             MANTRA~\cite{mantra}
             & 45.0 & 34.3 & 37.2 & 44.9 & 50.0 & 43.5 & 43.2 & 45.4
              \\
             QCNet~\cite{zhou2023query}
             & 46.1 & 35.5 & 35.7 & 46.2 & 51.1 & 44.5 & 44.1 & 46.4
              \\
              
            \midrule
             DSA~\cite{chan2016anticipating} 
             & 46.7 & 38.4 & 46.6 & 39.9 & 46.8 & 46.4 & 47.2 & 46.8
             \\
             RRL~\cite{zeng2017agent}
             & 46.6 & 46.3 & 49.3 & 33.5 & 48.0 & 48.8 & 49.1 & 48.6
             \\
             
             \midrule
             BP~\cite{li2020gcn}
             & 17.7 & 13.9 & 9.4 & 14.4 & 22.1 & 14.2 &  12.6 & 16.6
             \\
             BCP~\cite{li2020make}
             & 33.7 & 20.7 & 24.5 & 37.8 & 36.0 & 32.2 & 31.8 & 33.4
             \\
             \midrule
            \bottomrule
        \end{tabular}
        % }
\caption{Scenario-based performance analysis on weather, road topology, and traffic density. Note that TD denotes traffic density.}     %%%%%% interactive+collision+obstacle+non-interactive
\label{table:attributes}
\end{table*}

\clearpage


\begin{figure*}[t!]
\centering
\includegraphics[width=1.0\textwidth]{./sup_Figure/Scenario-based_ROI.pdf}
\caption{\textbf{Scenario-based Risk Localization and Anticipation Analysis.} Object painted in red denotes the true risk and the green boxes denote the predicted risk.}
\label{scenario-based_roi}
\end{figure*}

\begin{figure*}[t!]
\centering
\includegraphics[width=1.0\textwidth]{./sup_Figure/Augment_Object_Representation.pdf}
\caption{\textbf{Qualitative results of comparing adding object state representations for the vision-based methods.}}
\label{augment_object_representation}
\end{figure*}


% \begin{table*}[t!]
%     \small
%     \centering
%     % \resizebox{\textwidth}{!}{
%         \begin{tabular}
%             {@{}l @{\;}@{\;} c @{\;}c @{\;}c @{\;}c @{\;} c @{\;} c @{\;}  c @{\;} c @{\;} c @{\;} c @{\;}  c @{\;}c @{\;}c @{\;}c @{\;}c @{\;}c @{\;}c @{\;}c @{\;}c @{\;}c @{\;}c @{\;} c @{\;}c @{\;}c @{\;}c @{\;}}
%             \toprule
%              \multirow{2}{*} {\begin{tabular}{@{\;}c@{\;}} \end{tabular}} & 
%              \multicolumn{3}{c}{Four-wheeler}  & 
%              \multicolumn{3}{c}{Two-wheeler}  & 
%              \multicolumn{3}{c}{Pedestrian}  & 
%              \multicolumn{3}{c}{Night}  & 
%              \multicolumn{3}{c}{Rainy}  & 
%              \multicolumn{3}{c}{4-way}   & 
%              \multicolumn{3}{c}{3-way} &
%              \multicolumn{3}{c}{Straight} &
%             \\
%             \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}\cmidrule(lr){17-19}\cmidrule(lr){20-22}\cmidrule(lr){23-25}
%             &
            
%              \begin{tabular}{c@{\;}}  1s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  2s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  3s\end{tabular} &
%              \begin{tabular}{c@{\;}}  1s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  2s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  3s\end{tabular} &
%              \begin{tabular}{c@{\;}}  1s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  2s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  3s\end{tabular} &
%              \begin{tabular}{c@{\;}}  1s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  2s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  3s\end{tabular} &
%              \begin{tabular}{c@{\;}}  1s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  2s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  3s\end{tabular} &
%              \begin{tabular}{c@{\;}}  1s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  2s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  3s\end{tabular} &
%              \begin{tabular}{c@{\;}}  1s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  2s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  3s\end{tabular} &
%              \begin{tabular}{c@{\;}}  1s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  2s \end{tabular} & 
%              \begin{tabular}{c@{\;}}  3s\end{tabular} &

%             \\
%              \toprule

%              Range 
%              & 0.0 & 1.0 & 2.0 & 3.0 & 4.0 & \\
%             \midrule
%              QCNet~\cite{zhou2023query}   
%              & 10.0 & 20.0 & 30.0 & 40.0 & 50.0 & 60.0 & ..
%               \\
%             \midrule
%              RRL~\cite{zeng2017agent}
%               &
%              \\
%              \midrule
%              BCP~\cite{li2020make}
%               & 
%              \\
%              \midrule
%              Average
%              & 
%              \\
%             \midrule
%             \bottomrule
%         \end{tabular}
% \caption{Scenario-based temporal consistency analysis on risk types, weather, and road topology. The temporal consistency is assessed during the final second before reaching the critical/collision point.}
% \label{table:consistency}
% \end{table*}

